YaART: Yet Another ART Rendering Technology

In the rapidly progressing field of generative models, the development of efficient and high-fidelity text-to-image diffusion systems represents a significant frontier. This study introduces YaART, a novel production-grade text-to-image cascaded diffusion model aligned to human preferences using Reinforcement Learning from Human Feedback (RLHF). During the development of YaART, we especially focus on the choices of the model and training dataset sizes, the aspects that were not systematically investigated for text-to-image cascaded diffusion models before. In particular, we comprehensively analyze how these choices affect both the efficiency of the training process and the quality of the generated images, which are highly important in practice. Furthermore, we demonstrate that models trained on smaller datasets of higher-quality images can successfully compete with those trained on larger datasets, establishing a more efficient scenario of diffusion models training. From the quality perspective, YaART is consistently preferred by users over many existing state-of-the-art models.

==> supmat/04_fid_sbs.tex <==
\section{FID and Human Evaluations}
\label{sup:fid_sbs}

Our research does not rely on the Fréchet Inception Distance (FID) metric for evaluating the quality of generated images due to its low correlation with human evaluation when a generative model already produces high-quality results. This limitation of the FID metric has been acknowledged in previous works (SD XL, ???) and our study aligns with these findings (see Figure {}).

Caption for figure: The evolution of FID scores and human assessment scores during the training of a 1.4B sized model on full dataset. Despite a consistent change in FID scores throughout the training process, there is no corresponding change in human evaluation scores, demonstrating the disconnect between the two metrics in assessing the quality of generated images.
